Six-loop $\varepsilon$ expansion study of three-dimensional $O(n)\times O(m)$ spin models

The Landau-Wilson field theory with $O(n)\times O(m)$ symmetry which describes the critical thermodynamics of frustrated spin systems with noncollinear and noncoplanar ordering is analyzed in $4 - \varepsilon$ dimensions within the minimal subtraction scheme in the six-loop approximation. The $\varepsilon$ expansions for marginal dimensionalities of the order parameter $n^H(m,4-\varepsilon)$, $n^-(m,4-\varepsilon)$, $n^+(m,4-\varepsilon)$ separating different regimes of critical behavior are extended up to $\varepsilon^5$ terms. Concrete series with coefficients in decimals are presented for $m=\{2, \dots, 6\}$. The \textit{diagram of stability} of nontrivial fixed points, including the chiral one, in $(m,n)$ plane is constructed by means of summing up of corresponding $\varepsilon$ expansions using various resummation techniques. Numerical estimates of the chiral critical exponents for several couples $\{m,n\}$ are also found. Comparative analysis of our results with their counterparts obtained earlier within the lower-order approximations and by means of alternative approaches is performed. It is confirmed, in particular, that in physically interesting cases $n=2, m=2$ and $n=2, m=3$ phase transitions into chiral phases should be first-order.

==> expansions/nc/m=2/heis_num.tex <==
\begin{eqnarray}\label{nc_heis_num_m=2_6l}
n^H(2,4-\varepsilon)=2-\varepsilon+1.2942\varepsilon^{2}-2.9372\varepsilon^{3}+8.4135\varepsilon^{4}-28.311\varepsilon^{5}+\bigo{\varepsilon^{6}}.
\end{eqnarray}

==> expansions/nc/m=2/minus_num.tex <==
\begin{eqnarray}\label{nc_-_num_m=2_6l}
n^-(2,4-\varepsilon)=2.2020-0.56905\varepsilon+0.98920\varepsilon^{2}-2.2786\varepsilon^{3}+6.5406\varepsilon^{4}-21.696\varepsilon^{5}+\bigo{\varepsilon^{6}},
\end{eqnarray}
% \begin{eqnarray}\label{nc_-_num_m=2_6l}
% n^-(2,4-\varepsilon)=2.20204-0.569048\varepsilon+0.989202\varepsilon^{2}-2.27858\varepsilon^{3}+6.54061\varepsilon^{4}-21.6959\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
% \end{eqnarray}

==> expansions/nc/m=2/plus_num.tex <==
\begin{eqnarray}\label{nc_+_num_m=2_6l}
n^+(2,4-\varepsilon)=21.798-23.431\varepsilon+7.0882\varepsilon^{2}-0.032098\varepsilon^{3}+4.2650\varepsilon^{4}-8.4436\varepsilon^{5}+\bigo{\varepsilon^{6}},
\end{eqnarray}
% \begin{eqnarray}\label{nc_+_num_m=2_6l}
% n^+(2,4-\varepsilon)=21.798-23.431\varepsilon+7.08816\varepsilon^{2}-0.0320983\varepsilon^{3}+4.26503\varepsilon^{4}-8.44356\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
% \end{eqnarray}

==> expansions/nc/m=3/heis_num.tex <==
\begin{eqnarray}\label{nc_heis_num_m=3_6l}
n^H(3,4-\varepsilon)=1.3333-0.66667\varepsilon+0.86283\varepsilon^{2}-1.9581\varepsilon^{3}+5.6090\varepsilon^{4}-18.874\varepsilon^{5}+\bigo{\varepsilon^{6}}.
\end{eqnarray}
% \begin{eqnarray}\label{nc_heis_num_m=3_6l}
% n^H(3,4-\varepsilon)=1.33333-0.666667\varepsilon+0.862825\varepsilon^{2}-1.9581\varepsilon^{3}+5.60901\varepsilon^{4}-18.874\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
% \end{eqnarray}

==> expansions/nc/m=3/minus_num.tex <==
\begin{eqnarray}\label{nc_-_num_m=3_6l}
n^-(3,4-\varepsilon)=1.5081-0.28162\varepsilon+0.58272\varepsilon^{2}-1.4192\varepsilon^{3}+4.0193\varepsilon^{4}-13.086\varepsilon^{5}+\bigo{\varepsilon^{6}},
\end{eqnarray}
% \begin{eqnarray}\label{nc_-_num_m=3_6l}
% n^-(3,4-\varepsilon)=1.50807-0.281622\varepsilon+0.582719\varepsilon^{2}-1.41922\varepsilon^{3}+4.01932\varepsilon^{4}-13.0859\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
% \end{eqnarray}

==> expansions/nc/m=3/plus_num.tex <==
\begin{eqnarray}\label{nc_+_num_m=3_6l}
n^+(3,4-\varepsilon)=32.492-33.719\varepsilon+11.100\varepsilon^{2}-2.1440\varepsilon^{3}+5.2756\varepsilon^{4}-8.4830\varepsilon^{5}+\bigo{\varepsilon^{6}},
\end{eqnarray}
% \begin{eqnarray}\label{nc_+_num_m=3_6l}
% n^+(3,4-\varepsilon)=32.4919-33.7184\varepsilon+11.1002\varepsilon^{2}-2.14402\varepsilon^{3}+5.27562\varepsilon^{4}-8.48302\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
% \end{eqnarray}

==> expansions/nc/m=4/heis_num.tex <==
\begin{eqnarray}\label{nc_heis_num_m=4_6l}
n^H(4,4-\varepsilon)=1.-0.5\varepsilon+0.647119\varepsilon^{2}-1.46858\varepsilon^{3}+4.20676\varepsilon^{4}-14.1555\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}

==> expansions/nc/m=4/minus_num.tex <==
\begin{eqnarray}\label{nc_-_num_m=4_6l}
n^-(4,4-\varepsilon)=1.21539-0.0606898\varepsilon+0.208594\varepsilon^{2}-0.754223\varepsilon^{3}+2.25853\varepsilon^{4}-6.66437\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}

==> expansions/nc/m=4/plus_num.tex <==
\begin{eqnarray}\label{nc_+_num_m=4_6l}
n^+(4,4-\varepsilon)=42.7846-43.9393\varepsilon+14.3793\varepsilon^{2}-2.9445\varepsilon^{3}+5.85886\varepsilon^{4}-8.3568\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}

==> expansions/nc/m=5/heis_num.tex <==
\begin{eqnarray}\label{nc_heis_num_m=5_6l}
n^H(5,4-\varepsilon)=0.8-0.4\varepsilon+0.517695\varepsilon^{2}-1.17486\varepsilon^{3}+3.36541\varepsilon^{4}-11.3244\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}

==> expansions/nc/m=5/minus_num.tex <==
\begin{eqnarray}\label{nc_-_num_m=5_6l}
n^-(5,4-\varepsilon)=1.07704+0.118814\varepsilon-0.380548\varepsilon^{2}+0.599249\varepsilon^{3}+1.80549\varepsilon^{4}-25.8714\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}

==> expansions/nc/m=5/plus_num.tex <==
\begin{eqnarray}\label{nc_+_num_m=5_6l}
n^+(5,4-\varepsilon)=52.923-54.1188\varepsilon+17.4122\varepsilon^{2}-3.29174\varepsilon^{3}+6.20428\varepsilon^{4}-8.26768\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}

==> expansions/nc/m=6/heis_num.tex <==
\begin{eqnarray}\label{nc_heis_num_m=6_6l}
n^H(6,4-\varepsilon)=0.666667-0.333333\varepsilon+0.431413\varepsilon^{2}-0.979052\varepsilon^{3}+2.80451\varepsilon^{4}-9.43699\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}

==> expansions/nc/m=6/minus_num.tex <==
\begin{eqnarray}\label{nc_-_num_m=6_6l}
n^-(6,4-\varepsilon)=1.01613+0.274861\varepsilon-2.51705\varepsilon^{2}+24.9723\varepsilon^{3}-152.011\varepsilon^{4}-3148.63\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}

==> expansions/nc/m=6/plus_num.tex <==
\begin{eqnarray}\label{nc_+_num_m=6_6l}
n^+(6,4-\varepsilon)=62.9839-64.2749\varepsilon+20.3254\varepsilon^{2}-3.42118\varepsilon^{3}+6.43071\varepsilon^{4}-8.22523\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}


==> expansions/nc/m=7/heis_num.tex <==
\begin{eqnarray}\label{nc_heis_num_m=7_6l}
n^H(7,4-\varepsilon)=0.571429-0.285714\varepsilon+0.369782\varepsilon^{2}-0.839187\varepsilon^{3}+2.40386\varepsilon^{4}-8.08885\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}

==> expansions/nc/m=7/united_num.tex <==
\begin{eqnarray}\label{nc_-_num_m=7_6l}
n^-(7,4-\varepsilon)=73.-74.4167\varepsilon+23.1698\varepsilon^{2}-3.42738\varepsilon^{3}+6.59183\varepsilon^{4}-8.22288\varepsilon^{5}+\bigo{\varepsilon^{6}}.\
\end{eqnarray}

==> expansions/nc/together.tex <==
\begin{align}\label{nc_together}
n^+(2,4-\varepsilon)=&21.798-23.431\varepsilon+7.0882\varepsilon^{2}-0.032098\varepsilon^{3}+4.2650\varepsilon^{4}-8.4436\varepsilon^{5}+\bigo{\varepsilon^{6}}, \nonumber\\
n^-(2,4-\varepsilon)=&2.2020-0.56905\varepsilon+0.98920\varepsilon^{2}-2.2786\varepsilon^{3}+6.5406\varepsilon^{4}-21.696\varepsilon^{5}+\bigo{\varepsilon^{6}}, \nonumber\\
n^H(2,4-\varepsilon)=&2-\varepsilon+1.2942\varepsilon^{2}-2.9372\varepsilon^{3}+8.4135\varepsilon^{4}-28.311\varepsilon^{5}+\bigo{\varepsilon^{6}}, \nonumber\\
n^+(3,4-\varepsilon)=&32.492-33.719\varepsilon+11.100\varepsilon^{2}-2.1440\varepsilon^{3}+5.2756\varepsilon^{4}-8.4830\varepsilon^{5}+\bigo{\varepsilon^{6}},\nonumber\\
n^-(3,4-\varepsilon)=&1.5081-0.28162\varepsilon+0.58272\varepsilon^{2}-1.4192\varepsilon^{3}+4.0193\varepsilon^{4}-13.086\varepsilon^{5}+\bigo{\varepsilon^{6}},\nonumber\\
n^H(3,4-\varepsilon)=&1.3333-0.66667\varepsilon+0.86283\varepsilon^{2}-1.9581\varepsilon^{3}+5.6090\varepsilon^{4}-18.874\varepsilon^{5}+\bigo{\varepsilon^{6}}, \nonumber\\
n^+(4,4-\varepsilon)=&42.785-43.939\varepsilon+14.379\varepsilon^{2}-2.9445\varepsilon^{3}+5.8589\varepsilon^{4}-8.3568\varepsilon^{5}+\bigo{\varepsilon^{6}},\nonumber\\
n^-(4,4-\varepsilon)=&1.2154-0.060690\varepsilon+0.20859\varepsilon^{2}-0.75422\varepsilon^{3}+2.2585\varepsilon^{4}-6.6644\varepsilon^{5}+\bigo{\varepsilon^{6}},\nonumber\\
n^H(4,4-\varepsilon)=&1-0.5\varepsilon+0.64712\varepsilon^{2}-1.4686\varepsilon^{3}+4.2068\varepsilon^{4}-14.156\varepsilon^{5}+\bigo{\varepsilon^{6}},\nonumber\\
n^+(5,4-\varepsilon)=&52.923-54.119\varepsilon+17.412\varepsilon^{2}-3.2917\varepsilon^{3}+6.2043\varepsilon^{4}-8.2677\varepsilon^{5}+\bigo{\varepsilon^{6}},\nonumber\\
n^-(5,4-\varepsilon)=&1.0770+0.11881\varepsilon-0.38055\varepsilon^{2}+0.59925\varepsilon^{3}+1.8055\varepsilon^{4}-25.871\varepsilon^{5}+\bigo{\varepsilon^{6}},\nonumber\\
n^H(5,4-\varepsilon)=&0.8-0.4\varepsilon+0.51769\varepsilon^{2}-1.1749\varepsilon^{3}+3.3654\varepsilon^{4}-11.324\varepsilon^{5}+\bigo{\varepsilon^{6}},\nonumber\\
n^+(6,4-\varepsilon)=&62.984-64.275\varepsilon+20.325\varepsilon^{2}-3.4212\varepsilon^{3}+6.4307\varepsilon^{4}-8.2252\varepsilon^{5}+\bigo{\varepsilon^{6}},\nonumber\\
n^-(6,4-\varepsilon)=&1.0161+0.27486\varepsilon-2.5171\varepsilon^{2}+24.972\varepsilon^{3}-152.01\varepsilon^{4}-3148.63\varepsilon^{5}+\bigo{\varepsilon^{6}},\nonumber\\
n^H(6,4-\varepsilon)=&0.66667-0.33333\varepsilon+0.43141\varepsilon^{2}-0.97905\varepsilon^{3}+2.8045\varepsilon^{4}-9.4370\varepsilon^{5}+\bigo{\varepsilon^{6}}.\nonumber\\
\end{align}

==> sup/expansions/nc/m=2/minus.tex <==
\begin{eqnarray}
n^{+}&=&12+4\sqrt{6}+\varepsilon \left[-12-14\sqrt{\frac{2}{3}}\right]+\nonumber\\
&&+\varepsilon^{2}\left[\frac{137}{150}+\frac{91}{50}\frac{1}{\sqrt{6}}+\frac{13}{5}\zeta (3)+\frac{47}{10}\frac{1}{\sqrt{6}}\zeta (3)\right]+\nonumber\\
&&+\varepsilon^{3}\left[\frac{24257}{22500}+\frac{23369}{11250}\frac{1}{\sqrt{6}}+\frac{39}{20}\zeta (4)+\frac{47}{40}\sqrt{\frac{3}{2}}\zeta (4)\right.\nonumber\\
&&\left.\frac{3751}{4500}\zeta (3)+\frac{10621}{3000}\frac{1}{\sqrt{6}}\zeta (3)-\frac{232}{45}\zeta (5)-\frac{107}{15}\frac{1}{\sqrt{6}}\zeta (5)\right]+\nonumber\\
&&+\varepsilon^{4}\left[\frac{10272797}{27000000}+\frac{14010773}{27000000}\frac{1}{\sqrt{6}}+\frac{3751}{6000}\zeta (4)+\frac{10621}{4000}\frac{1}{\sqrt{6}}\zeta (4)\right.\nonumber\\
&&-\frac{21589597}{5400000}\zeta (3)-\frac{29909737}{3600000}\frac{1}{\sqrt{6}}\zeta (3)-\frac{58}{9}\zeta (6)-\frac{107}{12}\frac{1}{\sqrt{6}}\zeta (6)\nonumber\\
&&\frac{688433}{108000}\zeta (5)+\frac{245291}{24000}\frac{1}{\sqrt{6}}\zeta (5)-\frac{36911}{45000}\zeta (3)^2-\frac{268373}{120000}\frac{1}{\sqrt{6}}\zeta (3)^2\nonumber\\
&&\left.\frac{16317}{1600}\zeta (7)+\frac{5831}{3200}\sqrt{\frac{3}{2}}\zeta (7)\right]+\nonumber\\
&&+\varepsilon^{5}\left[\frac{53742149}{1012500000}-\frac{1360439947}{8100000000}\frac{1}{\sqrt{6}}-\frac{21589597}{7200000}\zeta (4)\right.\nonumber\\
&&-\frac{29909737}{4800000}\frac{1}{\sqrt{6}}\zeta (4)+\frac{618233}{86400}\zeta (6)+\frac{217091}{19200}\frac{1}{\sqrt{6}}\zeta (6)\nonumber\\
&&-\frac{196077}{50000}\zeta(3,5)+\frac{21859019}{800000}\zeta (8)+\frac{3834129}{1600000}\sqrt{\frac{3}{2}}\zeta (8)\nonumber\\
&&\frac{32793}{100000}\sqrt{\frac{3}{2}}\zeta(3,5)+\frac{1052267}{6750000}\zeta (3)+\frac{65775197}{27000000}\frac{1}{\sqrt{6}}\zeta (3)\nonumber\\
&&-\frac{36911}{30000}\zeta (4)\zeta (3)-\frac{268373}{80000}\frac{1}{\sqrt{6}}\zeta (4)\zeta (3)+\frac{24016567}{27000000}\zeta (3)^2\nonumber\\
&&\frac{1961931}{2000000}\sqrt{\frac{3}{2}}\zeta (3)^2-\frac{8551}{6750}\zeta (3)^3+\frac{3433}{7500}\frac{1}{\sqrt{6}}\zeta (3)^3\nonumber\\
&&\frac{9368587}{10800000}\zeta (5)-\frac{96653699}{21600000}\frac{1}{\sqrt{6}}\zeta (5)-\frac{41093}{11250}\zeta (3)\zeta (5)\nonumber\\
&&-\frac{59899573}{4320000}\zeta (7)-\frac{1357423}{320000}\sqrt{\frac{3}{2}}\zeta (7)+\frac{439829}{45000}\frac{1}{\sqrt{6}}\zeta (3)\zeta (5)\nonumber\\
&&\left.-\frac{12844009}{486000}\zeta (9)+\frac{3267247}{540000}\frac{1}{\sqrt{6}}\zeta (9)\right]+\bigo{\varepsilon^{6}}\nonumber\\
\end{eqnarray}


==> sup/expansions/nc/m=2/plus.tex <==
\begin{eqnarray}
n^{+}&=&12+4\sqrt{6}+\varepsilon \left(-12-14\sqrt{\frac{2}{3}}\right)+\nonumber\\
&&+\varepsilon^{2}\left(\frac{137}{150}+\frac{91}{50}\frac{1}{\sqrt{6}}+\frac{13}{5}\zeta (3)+\frac{47}{10}\frac{1}{\sqrt{6}}\zeta (3)\right)+\nonumber\\
&&+\varepsilon^{3}\left(\frac{24257}{22500}+\frac{23369}{11250}\frac{1}{\sqrt{6}}+\frac{39}{20}\zeta (4)+\frac{47}{40}\sqrt{\frac{3}{2}}\zeta (4)\right.\nonumber\\
&&\left.\frac{3751}{4500}\zeta (3)+\frac{10621}{3000}\frac{1}{\sqrt{6}}\zeta (3)-\frac{232}{45}\zeta (5)-\frac{107}{15}\frac{1}{\sqrt{6}}\zeta (5)\right)+\nonumber\\
&&+\varepsilon^{4}\left(\frac{10272797}{27000000}+\frac{14010773}{27000000}\frac{1}{\sqrt{6}}+\frac{3751}{6000}\zeta (4)+\frac{10621}{4000}\frac{1}{\sqrt{6}}\zeta (4)\right.\nonumber\\
&&-\frac{21589597}{5400000}\zeta (3)-\frac{29909737}{3600000}\frac{1}{\sqrt{6}}\zeta (3)-\frac{58}{9}\zeta (6)-\frac{107}{12}\frac{1}{\sqrt{6}}\zeta (6)\nonumber\\
&&\frac{688433}{108000}\zeta (5)+\frac{245291}{24000}\frac{1}{\sqrt{6}}\zeta (5)-\frac{36911}{45000}\zeta (3)^2-\frac{268373}{120000}\frac{1}{\sqrt{6}}\zeta (3)^2\nonumber\\
&&\left.\frac{16317}{1600}\zeta (7)+\frac{5831}{3200}\sqrt{\frac{3}{2}}\zeta (7)\right)+\nonumber\\
&&+\varepsilon^{5}\left(\frac{53742149}{1012500000}-\frac{1360439947}{8100000000}\frac{1}{\sqrt{6}}-\frac{21589597}{7200000}\zeta (4)\right.\nonumber\\
&&-\frac{29909737}{4800000}\frac{1}{\sqrt{6}}\zeta (4)+\frac{618233}{86400}\zeta (6)+\frac{217091}{19200}\frac{1}{\sqrt{6}}\zeta (6)\nonumber\\
&&-\frac{196077}{50000}\zeta(3,5)+\frac{21859019}{800000}\zeta (8)+\frac{3834129}{1600000}\sqrt{\frac{3}{2}}\zeta (8)\nonumber\\
&&\frac{32793}{100000}\sqrt{\frac{3}{2}}\zeta(3,5)+\frac{1052267}{6750000}\zeta (3)+\frac{65775197}{27000000}\frac{1}{\sqrt{6}}\zeta (3)\nonumber\\
&&-\frac{36911}{30000}\zeta (4)\zeta (3)-\frac{268373}{80000}\frac{1}{\sqrt{6}}\zeta (4)\zeta (3)+\frac{24016567}{27000000}\zeta (3)^2\nonumber\\
&&\frac{1961931}{2000000}\sqrt{\frac{3}{2}}\zeta (3)^2-\frac{8551}{6750}\zeta (3)^3+\frac{3433}{7500}\frac{1}{\sqrt{6}}\zeta (3)^3\nonumber\\
&&\frac{9368587}{10800000}\zeta (5)-\frac{96653699}{21600000}\frac{1}{\sqrt{6}}\zeta (5)-\frac{41093}{11250}\zeta (3)\zeta (5)\nonumber\\
&&-\frac{59899573}{4320000}\zeta (7)-\frac{1357423}{320000}\sqrt{\frac{3}{2}}\zeta (7)+\frac{439829}{45000}\frac{1}{\sqrt{6}}\zeta (3)\zeta (5)\nonumber\\
&&\left.-\frac{12844009}{486000}\zeta (9)+\frac{3267247}{540000}\frac{1}{\sqrt{6}}\zeta (9)\right)+\bigo{\varepsilon^{11/2}}\nonumber\\
\end{eqnarray}


==> tables/nc/all_pade.tex <==
\begin{table}[h!]
  \begin{center}
    \caption{Pad\'e estimates of $n^+$, $n^-$, $n^H$ for $m={2,\dots,7}$} %
    \label{tab:table1}
    \begin{tabular}{l|S|l|l|l|l|l|l}
      \textbf{m} & \textbf{order}& \textbf{2} & \textbf{3}& \textbf{4}& \textbf{5}& \textbf{6}& \textbf{7}\\
      \hline
      \hline
      \multirow{9}{*}{$n^+$} & 4-th &$4.6(2.0)$ &$7.70(1.26)$ &$10.3(1.5)$& $12.9(1.9)$& $15.3(2.6)$ & \\
                             & 4-th(B) &$5.35(14)$ &$8.59(63)$ & &&&\\
                             & 4-th(BI) &$5.35(14) $ &$8.62(74)$ & &&&\\
                             & 5-th &$5.25(83)$ &$8.9(1.8)$& $11.7(2.2)$& $14.6(2.4)$ &$17.3(2.5)$ & \\
                             & 5-th(B) &$5.6(1.1)$ & $8.72(32)$& &&&\\
                             & 5-th(BI) &$5.31(98)$ &$8.62(35)$ & &&&\\
                             & 6-th &$5.77(74)$ &$9.22(46)$ & $12.17(51)$&$14.99(53)$&$17.75(53)$&$20.47(52)$\\
                             & 6-th(B) &$6.15(19)$ & $9.333(88)$& &&&\\
                             & 6-th(BI) &$5.73(44)$ &$9.28(22) $ & &&&\\
      \hline
      \hline
        \multirow{3}{*}{$n^-$} & 4-th &$1.954(85)$ &$1.403(29)$&$1.2005(26)$ &$1.069(79)$&$1.055(25)$&\\
                             & 5-th &$1.948(55)$ & $1.401(20)$   & $1.191(36)$ &$1.066(69)$&$1.055(10)$&\\
                             & 6-th &$1.9690(87)$ &$1.4085(39)$&$1.1801(16)$ &$1.091(16)$&$1.067(21)$ &\\    
      \hline
      \hline
      \multirow{3}{*}{$n^H$} & 4-th &$1.47(21)$ & $0.98(14)$ &$0.73(11)$ & $0.588(86)$& $0.490(71)$&$0.420(61)$\\
                             & 5-th & $1.471(52)$ &$0.980(35)$ &$0.735(26)$&$0.588(21)$&$0.490(17)$ & $0.420(15)$\\
                             & 6-th &$1.474(38)$ &$0.983(25)$ & $0.737(19)$ &$0.590(15)$&$0.491(13)$&$0.421(11)$\\    
      \hline
    \end{tabular}
  \end{center}
\end{table}

==> tables/nc/all_pbl.tex <==
\begin{table}[h!]
  \begin{center}
    \caption{Pad\'e estimates of $n^+$, $n^-$, $n^H$ for $m={2,\dots,7}$} %
    \label{tab:table2}
    \begin{tabular}{l|S|l|l|l|l|l|l}
      \textbf{m} & \textbf{order}& \textbf{2} & \textbf{3}& \textbf{4}& \textbf{5}& \textbf{6}& \textbf{7}\\
      \hline
      \hline 
      \multirow{7}{*}{$n^+$} & 4-th &$\underset{(b=15)}{4.6(2.1)}$ &$\underset{(b=15)}{7.7(1.4)}$ &$\underset{(b=15)}{10.3(1.6)}$      & $\underset{(b=15)}{12.8(2.1)}   $& $\underset{(b=15)}{15.3(2.8)}$& \\
                             & 5-th &$\underset{(b=2.07)}{5.31(72)}$ &$\underset{(b=0.56)}{8.4(1.1)}$& $\underset{(b=0.64)}{11.2(1.3)}$& $\underset{(b=1.06)}{13.9(1.5)}$ & $\underset{(b=15)}{16.6(1.7)}$&\\
                             & 5-th(B) &$ $ & $\underset{(b=0)}{8.87(52)}$& &&&\\
                             & 5-th(BI) &$\underset{(b=1.2)}{6.50(54)}$ &$\underset{(b=0)}{8.3(0.9)}   $ & &&&\\
                             & 6-th &$\underset{(b=1.02)}{5.83(79)}$   &$\underset{(b=15)}{9.32(54)}   $ & $\underset{(b=15)}{12.26(56)}$&$\underset{(b=2.51)}{14.90(60)}$&$\underset{(b=3.52)}{17.68(64)}$&$\underset{(b=4.73)}{20.43(68)}$\\
                             & 6-th(B)  &$\underset{(b=15)}{6.12(36)}$ &$\underset{(b=15)}{9.10(36)}   $ & &&&\\
                             & 6-th(BI) &$\underset{(b=15)}{6.1(1)}$   &$\underset{(b=1.79)}{9.66(96)} $ & &&&\\
      \hline
      \hline
        \multirow{3}{*}{$n^-$}& 4-th &$\underset{(b=1.08)}{1.96809(9)}$ &$\underset{(b=3.65)}{1.40897(1)}  $&$-$                            &$\underset{(b=15)}{1.067(84)}$&$\underset{(b=9.99)}{1.04513(1)}$&\\
                              & 5-th &$\underset{(b=1.06)}{1.96821(4)}$ & $\underset{(b=3.14)}{1.41002(1)} $&$\underset{(b=15)}{1.185(30)}$ &$\underset{(b=15)}{1.064(71)}$&$\underset{(b=9.99)}{1.045125(1)}$&\\
                              & 6-th &$\underset{(b=2.68)}{1.97091(2)}$ &$\underset{(b=3.14)}{1.410021(1)} $&$\underset{(b=15)}{1.184(14)}$ &$\underset{(b=0)}{1.0867(95)}$&$--$ &\\    
      \hline
      \hline
            \multirow{3}{*}{$n^H$} & 4-th &$\underset{(b=0)}{1.480(54)}$ & $\underset{(b=0)}{0.986(36)}$ &$\underset{(b=0)}{0.740(27)}$ & $\underset{(b=0)}{0.592(22)}$& $\underset{(b=0)}{0.493(18)}$&$ \underset{(b=0)}{0.423(15)}$\\
                             & 5-th & $\underset{(b=1.19)}{1.454(13)}$ &$\underset{(b=1.19)}{0.9692(86)}$ &$\underset{(b=1.19)}{0.7269(65)}$&$\underset{(b=1.19)}{0.5815(52)}$&$\underset{(b=1.19)}{0.4846(43)}$ & $\underset{(b=1.19)}{0.4154(37)}$\\
                             & 6-th &$\underset{(b=1.85)}{1.4575(17)}$ &$\underset{(b=1.85)}{0.9717(11)}$ & $\underset{(b=1.85)}{0.72874(84)}$ &$\underset{(b=1.85)}{0.58299(67)}$&$\underset{(b=1.85)}{0.48583(56)}$&$\underset{(b=1.85)}{0.41642(48)}$\\    
      \hline
    \end{tabular}
  \end{center}
\end{table}


% \underset{(b=)}{}


==> tables/nc/pade_pbl.tex <==
\begin{table}[h!]
  \begin{center}
    \caption{Pad\'e estimates of $n^+$, $n^-$, $n^H$ for $m={2,\dots,7}$} %
    \label{tab:table1}
    \begin{tabular}{l|S|c|c|c|c|c|c}
      \textbf{m} & \textbf{order}& \textbf{2} & \textbf{3}& \textbf{4}& \textbf{5}& \textbf{6}& \textbf{7}\\
      \hline
      \hline
      \multirow{17}{*}{$n^+$} & 4-th &$4.6(2.0)$ &$7.70(1.26)$ &$10.3(1.5)$& $12.9(1.9)$& $15.3(2.6)$ & \\
                             & 4-th_B &$\underset{(b=15)}{4.6(2.1)}$ &$\underset{(b=15)}{7.7(1.4)}$ &$\underset{(b=15)}{10.3(1.6)}$      & $\underset{(b=15)}{12.8(2.1)}   $& $\underset{(b=15)}{15.3(2.8)}$& \\
                             & 4-th(B) &$5.35(14)$ &$8.59(63)$ & &&&\\
                             & 4-th(BI) &$5.35(14) $ &$8.62(74)$ & &&&\\
                             & 5-th &$5.25(83)$ &$8.9(1.8)$& $11.7(2.2)$& $14.6(2.4)$ &$17.3(2.5)$ & \\
                             & 5-th_B &$\underset{(b=2.07)}{5.31(72)}$ &$\underset{(b=0.56)}{8.4(1.1)}$& $\underset{(b=0.64)}{11.2(1.3)}$& $\underset{(b=1.06)}{13.9(1.5)}$ & $\underset{(b=15)}{16.6(1.7)}$&\\
                             & 5-th(B) &$5.6(1.1)$ & $8.72(32)$& &&&\\
                             & 5-th(B)_B &$- $ & $\underset{(b=0)}{8.87(52)}$& &&&\\
                             & 5-th(BI) &$5.31(98)$ &$8.62(35)$ & &&&\\
                             & 5-th(BI)_B &$\underset{(b=1.2)}{6.50(54)}$ &$\underset{(b=0)}{8.3(0.9)}   $ & &&&\\
                             & 6-th &$5.77(74)$ &$9.22(46)$ & $12.17(51)$&$14.99(53)$&$17.75(53)$&$20.47(52)$\\
                             & 6-th_B &$\underset{(b=1.02)}{5.83(79)}$   &$\underset{(b=15)}{9.32(54)}$& $\underset{(b=15)}{12.26(56)}$&$\underset{(b=2.51)}{14.90(60)}$&$\underset{(b=3.52)}{17.68(64)}$&$\underset{(b=4.73)}{20.43(68)}$\\
                             & 6-th(B) &$6.15(19)$ & $9.333(88)$& &&&\\
                             & 6-th(B)_B  &$\underset{(b=15)}{6.12(36)}$ &$\underset{(b=15)}{9.10(36)}   $ & &&&\\
                             & 6-th(BI) &$5.73(44)$ &$9.28(22) $ & &&&\\
                             & 6-th(BI)_B &$\underset{(b=15)}{6.1(1)}$   &$\underset{(b=1.79)}{9.66(96)} $ & &&&\\
                             & 6-th_{CB} &$6.02(56)$&$9.33(41)$ &$12.35(34)$ &$15.20(38)$ &$18.00(45)$&\\
      \hline
      \hline
        \multirow{6}{*}{$n^-$} & 4-th &$1.954(85)$ &$1.403(29)$&$1.2005(26)$ &$1.069(79)$&$1.055(25)$&\\
                               & 4-th_B &$\underset{(b=1.08)}{1.96809(9)}$ &$\underset{(b=3.65)}{1.40897(1)}  $&$-$                            &$\underset{(b=15)}{1.067(84)}$&$\underset{(b=9.99)}{1.04513(1)}$&\\
                               & 5-th &$1.948(55)$ & $1.401(20)$   & $1.191(36)$ &$1.066(69)$&$1.055(10)$&\\
                               & 5-th_B &$\underset{(b=1.06)}{1.96821(4)}$ & $\underset{(b=3.14)}{1.41002(1)} $&$\underset{(b=15)}{1.185(30)}$ &$\underset{(b=15)}{1.064(71)}$&$\underset{(b=9.99)}{1.045125(1)}$&\\
                               & 6-th &$1.9690(87)$ &$1.4085(39)$&$1.1801(16)$ &$1.091(16)$&$1.067(21)$ &\\    
                               & 6-th_B &$\underset{(b=2.68)}{1.97091(2)}$ &$\underset{(b=3.14)}{1.410021(1)} $&$\underset{(b=15)}{1.184(14)}$ &$\underset{(b=0)}{1.0867(95)}$&$-$ &\\
                               & 6-th_{CB} &$1.9704(36)$ &$1.406(11)$&$1.1824(85)$ &$-$&$-$ &\\
      \hline
      \hline
      \multirow{6}{*}{$n^H$} & 4-th &$1.47(21)$ & $0.98(14)$ &$0.73(11)$ & $0.588(86)$& $0.490(71)$&$0.420(61)$\\
                             & 4-th_B &$\underset{(b=0)}{1.480(54)}$ & $\underset{(b=0)}{0.986(36)}$ &$\underset{(b=0)}{0.740(27)}$ & $\underset{(b=0)}{0.592(22)}$& $\underset{(b=0)}{0.493(18)}$&$ \underset{(b=0)}{0.423(15)}$\\ 
                             & 5-th & $1.471(52)$ &$0.980(35)$ &$0.735(26)$&$0.588(21)$&$0.490(17)$ & $0.420(15)$\\
                             & 5-th_B & $\underset{(b=1.19)}{1.454(13)}$ &$\underset{(b=1.19)}{0.9692(86)}$ &$\underset{(b=1.19)}{0.7269(65)}$&$\underset{(b=1.19)}{0.5815(52)}$&$\underset{(b=1.19)}{0.4846(43)}$ & $\underset{(b=1.19)}{0.4154(37)}$\\
                             & 6-th &$1.474(38)$ &$0.983(25)$ & $0.737(19)$ &$0.590(15)$&$0.491(13)$&$0.421(11)$\\
                             & 6-th_B &$\underset{(b=1.85)}{1.4575(17)}$ &$\underset{(b=1.85)}{0.9717(11)}$ & $\underset{(b=1.85)}{0.72874(84)}$ &$\underset{(b=1.85)}{0.58299(67)}$&$\underset{(b=1.85)}{0.48583(56)}$&$\underset{(b=1.85)}{0.41642(48)}$\\    
                             & 6-th_{CB} &$\underset{(b=1.85)}{1.4575(17)}$ &$\underset{(b=1.85)}{0.9717(11)}$ & $\underset{(b=1.85)}{0.72874(84)}$ &$\underset{(b=1.85)}{0.58299(67)}$&$\underset{(b=1.85)}{0.48583(56)}$&$\underset{(b=1.85)}{0.41642(48)}$\\    
                             & 6-th_{CBH} &$\underset{(b=1.85)}{1.4575(17)}$ &$\underset{(b=1.85)}{0.9717(11)}$ & $\underset{(b=1.85)}{0.72874(84)}$ &$\underset{(b=1.85)}{0.58299(67)}$&$\underset{(b=1.85)}{0.48583(56)}$&$\underset{(b=1.85)}{0.41642(48)}$\\    
    \hline
    \end{tabular}
  \end{center}
\end{table}

